Termination of Rewriting on Reversible Boolean Circuits as a Free 3-Category Problem

Reversible Boolean Circuits are an interesting computational model under many aspects and in different fields, ranging from Reversible Computing to Quantum Computing. Our contribution is to describe a specific class of Reversible Boolean Circuits - which is as expressive as classical circuits - as a bi-dimensional diagrammatic programming language. We uniformly represent the Reversible Boolean Circuits we focus on as a free 3-category Toff. This formalism allows us to incorporate the representation of circuits and of rewriting rules on them, and to prove termination of rewriting. Termination follows from defining a non-identities-preserving functor from our free 3-category Toff into a suitable 3-category Move that traces the "moves" applied to wires inside circuits.

==> conclusion.tex <==
\section{Conclusion}
\label{section:Conclusion}
This work explores $3$-categories as a unified formal framework for modeling two concepts. First, it examines Reversible Boolean Circuits, which are treated as diagrams generated from a base through the iterative application of series/parallel compositions. Then, it investigates the termination of a rewriting system on these circuits.
\textbf{Toff} is the free $3$-category which effectively formalizes circuits and rewriting rules.
\textbf{Move} is the $3$-category supplying the well founded-order in a monoid of strings.
Termination follows from interpreting \textbf{Toff} into \textbf{Move} by means of a (strict) functor $\varphi$ that intuitively represent traces of moves inside the circuit being rewritten, by exploiting the common $3$-category structure.
A possible extension of this work is to evaluate its effectiveness in proving the termination of reductions of free $3$-polygraphs generated from alternative bases which include Fredkin and Peres gates.
A second development must focus on confluence: rewriting in \textbf{Toff} is not. We claim that the following circuits has two non-confluent normal forms:

\begin{center}
\begin{tikzcd}
\twocell{(sw *0 1) *1 (t2 *0 1) *1 (1 *0 sw) *1 (sw *0 1)}    \ \ \    \mbox{ (left-sliding)}
&
\twocell{(sw *0 1) *1 (1 *0 sw) *1 (sw *0 1) *1 (1 *0 t2)} \arrow[l,triple] \arrow[r,triple]
&
\mbox{ (permutation)}   \ \ \    \twocell{(1 *0 sw) *1 (sw *0 1) *1 (1 *0 sw) *1 (1 *0 t2)}
\enspace 
\end{tikzcd}
\end{center}

We are pursuing various directions in order to obtain confluence. However, the problem at hand is known to be non-obvious. Guiraud warns that a 3-polygraph may generate an infinite number of critical pairs which, in specific cases, can be categorized into a finite set of patterns, eventually leading to confluence \cite{GUIRAUD2006341}.


